Topics in Deep Learning and Optimization Algorithms for IoT Applications in Smart Transportation

Nowadays, the Internet of Things (IoT) has become one of the most important technologies which enables a variety of connected and intelligent applications in smart cities. The smart decision making process of IoT devices not only relies on the large volume of data collected from their sensors, but also depends on advanced optimization theories and novel machine learning technologies which can process and analyse the collected data in specific network structure. Therefore, it becomes practically important to investigate how different optimization algorithms and machine learning techniques can be leveraged to improve system performance. As one of the most important vertical domains for IoT applications, smart transportation system has played a key role for providing real-world information and services to citizens by making their access to transport facilities easier and thus it is one of the key application areas to be explored in this thesis. In a nutshell, this thesis covers three key topics related to applying mathematical optimization and deep learning methods to IoT networks. In the first topic, we propose an optimal transmission frequency management scheme using decentralized ADMM-based method in a IoT network and introduce a mechanism to identify anomalies in data transmission frequency using an LSTM-based architecture. In the second topic, we leverage graph neural network (GNN) for demand prediction for shared bikes. In particular, we introduce a novel architecture, i.e., attention-based spatial temporal graph convolutional network (AST-GCN), to improve the prediction accuracy in real world datasets. In the last topic, we consider a highway traffic network scenario where frequent lane changing behaviors may occur with probability. A specific GNN based anomaly detector is devised to reveal such a probability driven by data collected in a dedicated mobility simulator.

==> Introduction/introduction.tex <==

\textbf{Abstract:} In this chapter, we present an overview knowledge of the Internet of things and smart transportation as our research background. With these background, we highlight the research objective and key contributions. We organise this chapter as follows: in section \ref{overview} we introduce the Internet of things and smart transportation to readers as our work is based on this context; in section \ref{objectives} we discuss the research problems and objectives and highlight the research contributions in section \ref{contributions}; in section \ref{structure} we describe the thesis structure which matches with our research contributions in specific chapters.

\section{Overview}\label{overview}

Internet of Things (IoT) has played a key role in our daily life as it enables various intelligent applications in our cities. As one of the applications of IoT, which is most related to our daily travelling, smart transportation has served our citizens by offering real-world information and making transport facilities more convenient. Here we give a short background of IoT and smart transportation to provide a better scope that this thesis will cover.

\subsection{Internet of things} \label{IoTintro}
The Internet of Things (IoT) is a paradigm which is increasingly getting attention in modern wireless telecommunications. The basic concept of IoT is that ubiquitous objects around us, such as sensors and mobile phones, are able to communicate and cooperate with each other to solve a common problem \cite{giusto2010internet}. Specifically, the IoT network includes a variety of smart devices with the functions of connecting, exchanging and sharing data with each other over the Internet \cite{madakam2015internet}. In order to enable these functions in IoT networks, one of the key technologies is the Radio-Frequency IDentification (RFID) technology, which allows smart devices to exchange the information of device identification to the target receivers (e.g., Cloud facilities) by using RFID identifier \cite{jia2012rfid}. Another foundational technique is the wireless network used for connecting intelligent devices to monitor the environment. With these two techniques, an IoT system can capture real-time environmental data through sensors embedded in IoT devices. The data emitted from the system can be transmitted to the Cloud via gateways for further storage, process and analysis \cite{2011A}. Typically, in a cloud-dominant centralised architecture, Artificial Intelligence (AI) enabled computing nodes are often integrated and implemented at the cloud side, with an intention to collect the useful information from the transmitted data centrally and provide better insight for users to make decisions. Some recent IoT applications relying on this architecture are described in the following works, such as in the field of healthcare monitoring, traffic monitoring and environmental resource monitoring \cite{2018Brokering, 2018Economic, St2016Cloud, li2012compressed, he2012integration}. 

In a word, with the advances in wireless communication and sensor networks, IoT has been gaining attention in the area related to our daily life and more and more 'things' or smart objects are being involved in IoT networks. As a result, these IoT-related technologies have also made a large impact on new information and communications technology (ICT). However, the advanced IoT networks also come with inevitable shortcomings, especially those usually require the decision-making process to be conducted at the device side or edge side for better security \cite{9301390} and privacy protection \cite{9163078}.  Specifically, in a typical IoT scenario where data streams from various IoT devices can be transmitted to the Cloud and stored on a cloud database.  Our initial observation is that most IoT devices start to transmit data at a fixed transmission frequency, and such a transmission frequency is typically set by default or pre-defined by the device manufacturer with limited options made available to users. However, some advanced IoT devices with edge intelligence, e.g. Raspberry Pis and the Jetson series toolkit from Nvidia, can now be programmed to promptly respond to changes in the external environment \cite{10.1117/12.2571307, 8230004}, and can also be deployed with deep learning algorithms to satisfy stringent low-latency transmission requirements for time-sensitive IoT applications \cite{9287960, 9289509}. This approach does not sufficiently cater for a practical situation where groups of IoT devices may work collaboratively with limited system resources restricted by the operational environment. In fact, implementing IoT devices in a resource-constrained environment may impose two interesting problems in the design of IoT networks: 1) how to determine an adaptive transmission frequency for each IoT device so that an overall utility of the group of devices can be maximised in response to the dynamic changes of the environment; 2) how to ensure that different kinds of network resources can be better managed in a way that heterogeneous IoT devices can be engaged with the network in a secure, privacy-aware and plug-and-play manner. In order to address the mentioned problems, the first topic of this thesis is to propose a transmission frequency system for edge devices in an IoT network with a robust anomaly detection mechanism. 



%The Internet of Things (IoT) is a network including smart devices which can connect, exchange and share data with each other over the Internet \cite{madakam2015internet}. An IoT system can capture real-time environmental data through sensors embedded in IoT devices. The data emitted from the system can be transmitted to the Cloud via gateways for further storage, process and analysis \cite{2011A}. Typically, in a cloud-dominant centralised architecture, Artificial Intelligence (AI) enabled computing nodes are often integrated and implemented at the cloud side, with an intention to fetch the useful information from the transmitted data centrally and provide better insight for users to make decisions. Some recent IoT applications relying on this architecture are described in the following works \cite{2018Brokering, 2018Economic, St2016Cloud}. However, such an IoT system setup is highly dependent on the reliability of a remote cloud instance and often struggles to handle real-time data analysis and inference tasks with low latency requirements, e.g. anomaly detection. As a result, deploying AI on the edge, i.e., Edge AI, becomes more important for these tasks. Moreover, Edge AI provides an effective way for local edge devices to be engaged in such activities with better privacy awareness and enhanced system reliability, especially when a cloud instance could be delayed or fail in response in practical scenarios \cite{9301390, 9163078, atlam2020iot, zhou2014security}.

\subsection{Smart transportation} \label{smartcityinro}

%Nowadays, due to fast development in urbanisation, about 60 percent of the population lives around the city in the world and there are more and more people moving to cities every week \cite{chin2017understanding}. Therefore, the huge population and rapid industrialisation pose many challenges to traditional urban management. Unless we can refresh the urban style, it is unlikely that all human needs will be satisfied in the near future. 

On the one hand, IoT has played a key role in enabling the smart city, which combines data collection, analysis and decision making \cite{batty2012smart}. On the other hand, the smart city has become a terminology along with IoT, a novel city management approach to establish a collaborative society, where the data from daily life is leveraged to provide decisions for city management \cite{albino2015smart}.

Obviously, as the population is growing, the need for transportation increase dramatically and therefore smart transportation becomes the most challenging part of a smart city. To enable smart applications in modern transportation, advanced technologies, e.g. intelligent transportation system (ITS), have been proposed to provide creative insight for traffic management and improve user experience by providing proper information about the traffic network \cite{lin2017intelligent}. For instance, a smart parking system can save time for drivers, by informing drivers of the availability of parking spaces \cite{khanna2016iot}; carbon emissions and pollutants may also be minimised by recommending a shortest path to drivers for their parking search process \cite{agarana2017minimizing}. To sum up, smart transportation has shed a light on modern traffic management and satisfied the need of citizens in daily commuting. However, there are still open problems in smart transportation, such as traffic demand prediction, accident prevention, traffic flow prediction; cloud-based multi-agents planning; energy consumption \cite{rodrigue2020geography}, which are more challenging to deal with using conventional means of traffic management.

\subsubsection{Bike availability prediction}


As one of the common modes of transportation, bikes provide a healthy and convenient way for short-distance travel and sharing bikes have become prevalent in our cities. Also, an efficient bike-sharing system can not only reduce cost and commute time for urban commuters but also effectively mitigate the level of air pollution emissions generated in cities \cite{otero2018health}. 
However, bike availability prediction is one of the challenging problems in traffic demand prediction because the available number of bikes tends to be unbalanced, particularly at peak demand dates and hours \cite{hulot2018towards}. Therefore, an important consideration to make the bike-sharing system efficient is to balance supply and demand in the bike-sharing network \cite{raviv2013optimal}. To do this, traditional management methods such as manual monitoring systems, have been deployed to enable the relocation of bikes across different stations using other means of transportation, e.g. trucks \cite{7313194, raviv2013static}. However, this approach can easily lead to supply-demand imbalance due to estimation errors of system operators and unexpected traffic delays during the bike transition. Thus, due to the uncertainty of departure and arrival of bikes at any bike station, it is important to take a more proactive approach by accurately predicting the number of bikes that will be available for users to access at any given time and location. However, on the topic of traffic demand prediction, most of the work focus on taxi demand/availability prediction \cite{yao2018deep, yao2019revisiting} and limited work discusses the topic of availability prediction for sharing bike. Meanwhile, the current approaches are not able to forecast the availability precisely because of the weakness in traffic feature extraction and modelling. Therefore, in this thesis, the problem of sharing-bike availability prediction using graph neural network (GNN) is our second topic to discuss.


\subsubsection{Lane change detection}
As another challenge of smart transportation, accident prevention ensures driving safety and deserves more attention. Even if the traffic suggestions and regulations have been authorized to ensure a safe driving environment and minimise the chances of a traffic accident as much as possible, malicious driving intentions (e.g., acute acceleration; frequent lane changing) still play a threat to traffic safety and disturb the normal traffic flow. For instance, a speed advisory system (SAS) offers speed guidance for ensuring driving safety, but the vehicles tend to be driven with unexpected acceleration and lane changing behaviours \cite{jeon2014effects}, once they leave the road segment with SAS. Therefore, detection of driving intentions has been involved in traffic management, alarming for intervention when the driving safety may be under threat, such as traffic incidents\cite{asakura2017incident} \cite{hawas2007fuzzy}, traffic congestion \cite{wang2018locality} and malicious driving \cite{8886013}.
It is worth paying attention to frequent lane changing, which may easily result in severe traffic accidents on highway networks. Existing approaches, such as hidden Markov model (HMM) \cite{li2016lane} and LSTM-based methods \cite{tang2020driver, 8813987}, have been found less capable in dealing with the lane changing detection problems as they can not model the traffic data with natural geographical information (e.g, the connection between lanes) sufficiently. Therefore, the last topic in this thesis concerns the detection for lane changing intention using GNN to leverage the geographical information on the highway network, to improve the detection performance.



%\begin{itemize}
%	\item Traffic flow prediction.
%	\item Traffic demand prediction.
%	\item Cloud-based multi agents planning.
%	\item Accidents and safety.
%	\item Energy consumption.
%\end{itemize}



\section{Research objectives}\label{objectives}

\textbf{Research objectives 1:} Optimise transmission frequencies for edge devices in IoT network with robust anomaly detection mechanism.

We consider the two problems of the design of IoT networks, as discussed in section \ref{IoTintro}. Our key assumption is that different IoT devices may have different priority levels when transmitting data in a resource-constrained environment and that those priority levels may only be locally defined and accessible by edge devices for privacy concerns. With these in mind, the research objective is to optimise the transmission frequencies for a group of IoT edge devices under practical constraints. We aim at establishing a transmission frequency management system which can allocate optimal transmission frequencies to IoT devices and maximise the overall utility of the edge devices in the IoT network in a decentralised manner. In order to ensure the security of the system, we shall also devise an anomaly detector, on top of the designed optimal transmission management system, which can effectively identify abnormal transmission frequencies in different settings. The anomaly detector is expected to only leverage limited information from the IoT system. We will investigate both mathematical rule-based and deep learning based approaches, and examine their efficacy in tackling such challenges. 

%We consider the two problems of the design of IoT network, as discussed in section \ref{IoTintro}. The research objective is to to optimise the transmission frequencies for a group of IoT edge devices under practical constraints. Our key assumption is that different IoT devices may have different priority levels when transmitting data in a resource-constrained environment and that those priority levels may only be locally defined and accessible by edge devices for privacy concerns. To address the two research problems, we establish transmission frequency management system which can allocate the optimal transmission frequencies to IoT devices and maximise the system overall utility, by leveraging Alternating Direction Method of Multipliers (ADMM) optimisation method and demonstrating its applicability for effectively managing various IoT data streams in a decentralised framework. With the frequency management system, we devise an anomaly detector to detect different types of anomalies which can lead the IoT devices to transmit data stream under incorrect transmission frequencies. The anomaly detector only requires limited information from the IoT system, and can be operated using both a mathematical rule-based approach and the deep learning approach.

%Given the context where IoT devices transmit data under optimal transmission frequencies, we also design an anomaly detector which is able to find out any local device that \textit{implicitly} tampers its transmission frequency in real-time. It is important to note that we do not focus on the detection of anomalies in \textit{data contents}, e.g., changing a data entry in the transmitted json file from value ``A" to ``B" \cite{miller2016detection}, instead of we are interested in detecting the change of transmission frequency as a result of the anomalies happening on the edge devices.


\noindent \textbf{Research objectives 2:} Availability prediction for the sharing-bike scheme using spatial-temporal graph convolutional network. 

As to a research topic related to smart transportation, we first consider the problem of availability prediction for sharing bikes. The research objective is to present a availability prediction system which can forecast the available number of sharing bikes among different bike stations accurately and promptly using models trained on realistic data. In particular, spatial-temporal graph convolutional network (ST-GCN), as a powerful variant of graph convolutional networks (GCN) which aims to capture the relationship of data contained in the graphical nodes across both spatial and temporal dimensions, is applied for improving the prediction accuracy. Recently, graph based solutions have caught much attention in the literature as they have shown efficacy in improving traffic management. We shall apply spatial-temporal graph convolutional network (ST-GCN) to capture the relationship of data between graph nodes and compare its performance with other schemes to illustrate its efficacy in chapter \ref{bike}. Moreover, the impacts of different modelling methods of adjacency matrices shall be investigated.




\noindent \textbf{Research objectives 3:} Detecting lane changing intention on highway network scenario using graph neural network.

The last research objective is related to driving safety. As mentioned previously in section \ref{smartcityinro}, frequent lane changing intention threatens driving safety on the highway network. The objective of this part is to develop an algorithm which is able to detect the frequent lane changing behaviour on highway network using graph-based deep learning methods. As we shall see, the proposed algorithm will be able to forecast the lane changing probability of vehicles on a segment of the highway network in real-time.

%As the population grows in different cities, highway traffic network is playing an important role in modern transportation infrastructures. Although speed advisory system (SAS), as a part of intelligent transportation systems (ITS), provides assistance to manage the traffic flow in a highway traffic networks, driving safety is still under threat by different driving intentions like unexpected acceleration, deceleration and lane changes, which may cause the severe collisions on highway networks. In this paper, we detect traffic flow caused by lane changing intentions on the highway traffic networks, with graph modelling on the data generated by a popular mobility simulator. Given the different lengths of traffic flow data, we evaluate the performance of lane changing detection using the state-of-the-art model, attention temporal graph convolutional neural network (ATGCN) and compared the detection performance with temporal convolutional neural network (TCNN). Experiment results show that ATGCN has advantages in short-term detection and the lane changing intention can be detected promptly within 90 seconds with the highest accuracy $99.42\%$. We also analyse the features in the temporal and spectral domain, in order to illustrate the specific patterns which contribute more to lane changing detection.



\section{Thesis contributions}\label{contributions}
The thesis discusses three topics related to IoT and smart transportation. The contributions of the thesis can be summarised as followed:

\begin{itemize}
	\item In chapter \ref{IoT}, we propose a transmission frequency management system which is able to find the optimal transmission frequency for each IoT device, in order to maximise the overall utility in a resource-constrained, privacy-aware environment. Design an anomaly detector to ensure the transmission frequencies of the proposed IoT transmission frequency management system are in good order. 
	
	\item In chapter \ref{bike}, we design a deep learning architecture by combining attention mechanism with the spatial-temporal graph neural network, to better predict the sharing-bike availability based on realistic datasets. Furthermore, we also discuss the impacts of different modelling methods of adjacency matrices on the proposed architecture.
	
	
	\item In chapter \ref{lane}, we apply a refined version of a graph neural network, to predict the lane changing intention and analysis the pattern of driving data for the purpose of model interpretability.
	
\end{itemize}


\section{Thesis structure}\label{structure}

The thesis is organised as follows:

\begin{itemize}
	\item Chapter 1 introduces the background, our research objectives, thesis contribution and structure.
	\item Chapter 2 approaches the first research objective by applying optimisation and deep learning method to IoT systems.
	\item Chapter 3 achieves the second research objective by leveraging graph neural networks to forecast the sharing-bike availability, based on the data collected by IoT devices embedded in bike stations.
	\item Chapter 4 tackles the third research problem by using graph neural network to analyse the driving patterns and predict the lane changing intention, based on the data generated from a novel mobility simulator.
	\item Chapter 5 summarises the thesis and highlights the potential directions for future work.
\end{itemize}

%\section{Summary}\label{summary}
%
%In this chapter, we described the background knowledge of IoT and smart city for our research and we clarify  the three research objectives that this thesis intends to approach. Finally, we highlighted the thesis contributions and presented the thesis structure which is organised related to the three research objectives.


==> thanks/thanks.tex <==


To my family and Wenting Luo.

